Fully-Dynamic Decision Trees

We develop the first fully dynamic algorithm that maintains a decision tree over an arbitrary sequence of insertions and deletions of labeled examples. Given $\epsilon > 0$ our algorithm guarantees that, at every point in time, every node of the decision tree uses a split with Gini gain within an additive $\epsilon$ of the optimum. For real-valued features the algorithm has an amortized running time per insertion/deletion of $O\big(\frac{d \log^3 n}{\epsilon^2}\big)$, which improves to $O\big(\frac{d \log^2 n}{\epsilon}\big)$ for binary or categorical features, while it uses space $O(n d)$, where $n$ is the maximum number of examples at any point in time and $d$ is the number of features. Our algorithm is nearly optimal, as we show that any algorithm with similar guarantees uses amortized running time $\Omega(d)$ and space $\tilde{\Omega} (n d)$. We complement our theoretical results with an extensive experimental evaluation on real-world data, showing the effectiveness of our algorithm.

==> macros.tex <==
\newcommand{\scO}{\mathcal{O}}
\newcommand{\scA}{\mathcal{A}}
\newcommand{\scX}{\mathcal{X}}
\newcommand{\scE}{\mathcal{E}}
\newcommand{\scF}{\mathcal{F}}
\newcommand{\scY}{\mathcal{Y}}
\newcommand{\scD}{\mathcal{D}}
\newcommand{\scL}{\mathcal{L}}
\newcommand{\scN}{\mathcal{N}}
\newcommand{\scP}{\mathcal{P}}
\newcommand{\scQ}{\mathcal{Q}}
\newcommand{\scT}{\mathcal{T}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\bc}{\pmb{c}}
\newcommand{\ba}{\pmb{a}}
\newcommand{\bp}{\pmb{p}}
\newcommand{\bq}{\pmb{q}}
\newcommand{\bg}{\pmb{g}}
\newcommand{\bbf}{\mathbf{f}}
\newcommand{\bx}{\pmb{x}}
\newcommand{\br}{\pmb{r}}
\newcommand{\by}{\pmb{y}}
\newcommand{\bz}{\pmb{z}}
\newcommand{\bv}{\pmb{v}}
\newcommand{\Ind}{\mathds{1}}
\newcommand{\ED}{\triangle}
\newcommand{\EDR}{\ED^{\!*}}
\newcommand*\xor{\oplus}
\newcommand{\rt}{\operatorname{r}}
\newcommand{\norm}[2]{\| {#2} \|_{#1}}
\newcommand{\tvd}[1]{\norm{tvd}{#1}}
\newcommand{\evsplit}{\scE_{\operatorname{split}}}
\newcommand{\psplit}{p_{\operatorname{split}}}
\newcommand{\evstop}{{\operatorname{stop}}}
\newcommand{\pstop}{p_{\operatorname{stop}}}
\newcommand{\splitvar}{{\operatorname{split}}}
\newcommand{\splitdist}{P_{\operatorname{split}}}
\newcommand{\Tup}{T^{\uparrow}}
\newcommand{\Tdown}{T^{\downarrow}}
\newcommand{\up}[1]{{#1}^{\uparrow}}
\newcommand{\down}[1]{{#1}^{\downarrow}}
\newcommand{\mauro}[1]{{\color{blue} #1}}
\newcommand{\marco}[1]{{\color{red} #1}}
\newcommand{\softmax}{\operatorname{softmax}}

\newcommand{\shorteq}{%
%  \settowidth{\@tempdima}{-}% Width of hyphen
  \resizebox{4pt}{\height}{=}%
}
\newcommand{\Dev}{D}
